A benchmark for surface-tension-driven incompressible two-phase flows

The Volume-of-Fluid (VoF) method for simulating incompressible two-phase flows is widespread in academic and commercial simulation software because of its many advantages: a high degree of volume conservation, applicability to unstructured domain discretization (relevant for engineering applications), straightforward parallel implementation with the domain-decomposition and message-passing approach (important for large-scale simulations), and intrinsic handling of strong deformations and topological changes of the fluid interface. However, stable and accurate handling of small-scale capillary flows (dominated by surface tension forces) is still challenging for VoF methods. With many different VoF methods making their way into commercial and open-source software, it becomes increasingly important to compare them quantitatively and directly. For this purpose, we propose a set of simulation benchmarks and use them to directly compare VoF methods available in OpenFOAM, Basilisk, and Ansys Fluent. We use Jupyter notebooks to document and process the benchmark results, making a direct comparison of our results with other two-phase simulation methods very straightforward. The publicly available input data, secondary benchmark data, and post-processing Jupyter notebooks can be re-used by any two-phase flow simulation method that discretizes two-phase Navier-Stokes equations in a one-fluid formulation, which can save a significant amount of person-hours.

==> credit-statement.tex <==
\section*{CRediT author statement}

% INFO:
%* Conceptualization; formulation or evolution of overarching research goals and aims
%* Methodology: Development or design of methodology; creation of models
%* Software: Programming, software development; designing computer programs; implementation of the computer code and supporting algorithms; testing of existing code components
%* Validation: Verification, whether as a part of the activity or separate, of the overall replication/ reproducibility of results/experiments and other research outputs
%* Formal analysis: Application of statistical, mathematical, computational, or other formal techniques to analyze or synthesize study data
%* Investigation: Conducting a research and investigation process, specifically performing the experiments, or data/evidence collection
%* Resources: Provision of study materials, reagents, materials, patients, laboratory samples, animals, instrumentation, computing resources, or other analysis tools
%* Data Curation: Management activities to annotate (produce metadata), scrub data and maintain research data (including software code, where it is necessary for interpreting the data itself) for initial use and later reuse
%* Writing - Original Draft: Preparation, creation and/or presentation of the published work, specifically writing the initial draft (including substantive translation)
%* Writing - Review & Editing: Preparation, creation and/or presentation of the published work by those from the original research group, specifically critical review, commentary or revision – including pre-or postpublication stages
%* Visualization: Preparation, creation and/or presentation of the published work, specifically visualization/ data presentation
%* Supervision: Oversight and leadership responsibility for the research activity planning and execution, including mentorship external to the core team
%* Project administration: Management and coordination responsibility for the research activity planning and execution
%* Funding acquisition: Acquisition of the financial support for the project leading to this publication

\begin{description}

\item Anja Lippert: Conceptualization, Methodology, Software, Formal analysis, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization

\item Tobias Tolle: Conceptualization, Methodology, Software, Formal analysis, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization

\item Aaron Dörr: Conceptualization, Methodology, Software, Formal analysis, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization

\item Tomislav Maric: Conceptualization, Methodology, Formal analysis, Data Curation, Writing - Original Draft, Writing - Review \& Editing 

\end{description}

